DART: Disentanglement of Accent and Speaker Representation in Multispeaker Text-to-Speech

Recent advancements in Text-to-Speech (TTS) systems have enabled the generation of natural and expressive speech from textual input. Accented TTS aims to enhance user experience by making the synthesized speech more relatable to minority group listeners, and useful across various applications and context. Speech synthesis can further be made more flexible by allowing users to choose any combination of speaker identity and accent, resulting in a wide range of personalized speech outputs. Current models struggle to disentangle speaker and accent representation, making it difficult to accurately imitate different accents while maintaining the same speaker characteristics. We propose a novel approach to disentangle speaker and accent representations using multi-level variational autoencoders (ML-VAE) and vector quantization (VQ) to improve flexibility and enhance personalization in speech synthesis. Our proposed method addresses the challenge of effectively separating speaker and accent characteristics, enabling more fine-grained control over the synthesized speech. Code and speech samples are publicly available.

==> Sections/Discussion.tex <==
\section{Discussion}
\label{sec:discussion}

 Our proposed method focuses on disentangling speaker and accent characteristics, but there may be other factors affecting the synthesized speech quality, such as prosody, intonation, or speaking style. Future work should aim to develop approaches that encompass a broader range of speech attributes, enabling TTS systems to generate speech that is not only accentually accurate but also conveys the desired expressive qualities. Additionally, expanding the dataset and considering a wider range of speakers and accents would be valuable. The availability of more diverse and extensive training data can contribute to the generalization and robustness of the TTS models. Collecting and incorporating data from underrepresented accents or languages can help address biases and ensure inclusivity in synthesized speech.

%  The proposed CVAE model achieves promising results in terms of objective and subjective evaluation. As shown in Section~\ref{subsec:analysis}, the embedding space allows for strong accent conversion but this can come at the price of identity disruption. This accent-identity balance is a complex issue, as accent partially forms a person's identity. On this note, the baseline of GMVAE seems to have captured speaker identity too well, hence not allowing for a significant change in accent. We note that this issue might be amplified by the dataset only having 4 speakers per accent. In an extreme case, where one would have just 1 speaker per accent, it would not be possible to distinguish between accent and speaker identity at all. Finally, it is worth mentioning that the accent-identity balance preference can depend on the application. If the primary concern is to convert an audio for better intelligibility, then a change in identity can be a bearable downside; while in some applications, such as TTS for people with muteness, retaining speaker identity might be the more important aspect of the two. Ideally, speaker identity and accent should be completely disentangled.
% In future work, we aim to focus on designing stronger disentanglement mechanisms to better separate accent from speaker identity. 


%The L2Arctic dataset~\cite{zhao2018l2} is a very convenient dataset to use. However, another problem that accented TTS is facing, with the limited datasets that we have, is the accent intensity variance across speakers, i.e., the occurence of speakers whose accent sounds quite close to L1, and those whose accent is very non-native. This effect inconsistency is naturally amplified the lower the number of speakers in a dataset. Last point that can be limiting the current results is the speaker's language proficiency. In L2Arctic, a substantial portion of the samples contains little pauses that were most likely caused by the lack of speaker's language knowledge, resulting in them taking time to decide on how to pronounce certain words in the written prompts. We believe that addressing these two points would benefit accented TTS research. Another option is to collect and use a much wider dataset that would consist of many speakers in each accent.This problem should be addressed in the future through stronger disentanglement mechanisms.

%accent-speaker trade-off -> if we see it in the results...

==> Sections/Motivation.tex <==
\section{Motivation}
\textbf{This section would be good if it showed the embeddings and talked about how the SLT work inspired us... we just had other problems to solve first and weren't able to...}
Research and development in both accented TTS and accent conversion have the potential to enrich communication experiences, foster inclusivity, celebrate cultural diversity, and break down language barriers in our increasingly interconnected world.  Accented TTS research aims to enhance the inclusivity and accessibility of voice-based communication systems. By developing TTS systems that can accurately and naturally generate accents from various regions, we can bridge communication gaps and empower individuals who speak different languages or have diverse accents to express themselves more effectively.

In this work, we seek to advance the field of TTS technology by proposing innovative approaches to distinguish the speaker's identity from accent variations in synthesized speech. By disentangling these factors, we aim to achieve enhanced flexibility, control, and adaptability in generating speech with specific accents while maintaining the unique characteristics of the speaker. The potential impact of this research is significant across various applications, such as voice assistants, language learning tools, and entertainment media.

The main objective of this work is to explore a novel method for separating speaker identity and accent representation within the context of multispeaker TTS synthesis. Our investigation will focus on an existing deep probabilistic model called \encoder{} that has demonstrated proficiency in learning a disentangled representation of a set of grouped observations. To achieve this disentanglement, we will leverage the \encoder{}, which operates at both the group level and the observation level, effectively separating the latent representation into semantically meaningful components. Furthermore, this approach allows for efficient test-time inference, ensuring practical applicability.
